Explaining Control Policies through Predicate Decision Diagrams

Safety-critical controllers of complex systems are hard to construct manually. Automated approaches such as controller synthesis or learning provide a tempting alternative but usually lack explainability. To this end, learning decision trees (DTs) have been prevalently used towards an interpretable model of the generated controllers. However, DTs do not exploit shared decision-making, a key concept exploited in binary decision diagrams (BDDs) to reduce their size and thus improve explainability. In this work, we introduce predicate decision diagrams (PDDs) that extend BDDs with predicates and thus unite the advantages of DTs and BDDs for controller representation. We establish a synthesis pipeline for efficient construction of PDDs from DTs representing controllers, exploiting reduction techniques for BDDs also for PDDs.

==> tables/decision_ablation.tex <==
% !TEX root =  ../main.tex

\begin{table*}[h!]
	\centering
	\caption{Number of decision nodes in the PDDs generated in each step of the pipeline}
	\setlength{\tabcolsep}{7pt}
	\begin{adjustbox}{width=.7\textwidth,center}
		%\resizebox{1.15\textwidth}{!}{
			\begin{tabular}{l|rrrrr}
				\toprule
				   & DT & BDD & & Consistency & Care-set\\			
				Controllers & learning & compilation & Reordering & transformation & reduction\\
				\toprule
				10rooms	& 8648	& 1332	& 419	& 344	& 344\\
				cartpole	& 126	& 206	& 172	& 133	& 126\\
				cruise-latest	& 493	& 1091	& 554	& 479	& 476\\
				dcdc	& 135	& 149	& 135	& 135	& 135\\
				helicopter	& 3169	& 10294	& 5577	& 3276	& 3158\\
				traffic\_30m	& 6286	& 11088	& 5461	& 2497	& 2350\\
				\midrule
				beb.3-4.LineSeized	& 32	& 33	& 32	& 32	& 32\\
				blocksworld.5	& 617	& 2646	& 1742	& 1526	& 796\\
				cdrive.10	& 1200	& 9442	& 3828	& 3828	& 1200\\
				consensus.2.disagree	& 33	& 48	& 36	& 33	& 31\\
				csma.2-4.some\_before	& 51	& 78	& 60	& 58	& 53\\
				eajs.2.100.5.ExpUtil	& 83	& 108	& 81	& 81	& 85\\
				echoring.MaxOffline1	& 934	& 4429	& 1288	& 1274	& 970\\
				elevators.a-11-9	& 8163	& 16563	& 6126	& 6077	& 5555\\
				exploding-blocksworld.5	& 2490	& 14857	& 6648	& 6504	& 3635\\
				firewire\_abst.3.rounds	& 12	& 12	& 12	& 12	& 12\\
				ij.10	& 645	& 458	& 452	& 452	& 453\\
				pacman.5	& 21	& 28	& 23	& 23	& 21\\
				philosophers-mdp.3	& 195	& 310	& 246	& 205	& 203\\
				pnueli-zuck.5	& 85685	& 1304402	& 496033	& 73139	& 72192\\
				rabin.3	& 55	& 80	& 62	& 59	& 58\\
				rectangle-tireworld.11	& 240	& 281	& 274	& 240	& 240\\
				triangle-tireworld.9	& 13	& 14	& 14	& 13	& 13\\
				wlan\_dl.0.80.deadline	& 1684	& 13763	& 3513	& 2004	& 1824\\
				zeroconf.1000.4.true.correct\_max	& 41	& 60	& 55	& 56	& 44\\
				\bottomrule    
			\end{tabular}
		\end{adjustbox}
		\label{table:decision-nodes-ablation}
	\end{table*}

==> tables/nodes-comparison.tex <==
% !TEX root =  ../main.tex

\begin{table*}[h!]
		\centering
		\caption{Number of decision nodes in representations of controllers. The upper part of the table contains permissive policies from \scots\ and \uppaal, while the lower part contains deterministic policies from \storm. ``States'' is the number of states in the controller. {\#}shared denoted the number of shared nodes in the PDD. The DTs are generated using \dtcontrol\ with entropy impurity measure, axis-aligned predicates, without early-stopping. The smallest size in each row is written in bold.\\ }
	\setlength{\tabcolsep}{7pt}
	\begin{adjustbox}{width=.7\textwidth,center}
	%\resizebox{1.15\textwidth}{!}{
	\begin{tabular}{l|rrrr|r|S[table-format=-1.2,table-align-text-post=false]S[table-format=-1.2,table-align-text-post=false]S[table-format=-1.2,table-align-text-post=false]H}%use H if you want to hide a column % to highlight a column >{\columncolor[gray]{0.9}}
		\toprule
%		&& bit-blasted &&&&&\\
Controllers              & States & bbBDD & DT & PDD & {\#}shared &	$\frac{\mathit{DT}}{\mathit{bbBDD}}$ & $\frac{\mathit{PDD}}{\mathit{bbBDD}}$	&	$\frac{\mathit{PDD}}{\mathit{DT}}$	&	$\frac{\mathit{DT}}{\mathit{BDD}}$\\[1mm] %Note: I have hidden the last column
		\toprule
		10rooms                 & 26244    & 1102           & 8648          & \textbf{344}   & 211 & 7.85 & 0.31 & 0.04 & 7.85 \\
		cartpole                & 271      & 197            & \textbf{126}  & \textbf{126}   & 0 & 0.64 & 0.64 & 1    & 0.64 \\
		cruise-latest           & 295615   & 2115           & 493           & \textbf{476}   & 66 & 0.23 & 0.23 & 0.97 & 0.23 \\
		dcdc                    & 593089   & 814            & \textbf{135}  & \textbf{135}  & 0  & 0.17 & 0.17 & 1    & 0.17 \\
		helicopter              & 280539   & 3348           & 3169          & \textbf{3158}  & 486 & 0.95 & 0.94 & 1    & 0.95 \\
		traffic\_30m            & 16639662 & 4522           & 6286          & \textbf{2350}  & 1538 & 1.39 & 0.52 & 0.37 & 1.39 \\ 
%		truck{\textunderscore}trailer	&	1386211 & 	&	TO	&		&		&		&	\\
		\midrule
		beb.3-4.LineSeized      & 4173     & 1051           & \textbf{32}   & \textbf{32}   & 0  & 0.03 & 0.03 & 1    & 0.03 \\
		blocksworld.5           & 1124     & 4043           & \textbf{617}  & 796            & 13 & 0.15 & 0.2  & 1.29 & 0.15 \\
		cdrive.10               & 1921     & 6151           & \textbf{1200} & \textbf{1200}  & 0 & 0.2  & 0.2  & 1    & 0.2  \\
		consensus.2.disagree    & 2064     & 112            & 33            & \textbf{31}    & 1 & 0.29 & 0.28 & 0.94 & 0.29 \\
		csma.2-4.some\_before   & 7472     & 1172           & \textbf{51}   & 53             & 2 & 0.04 & 0.05 & 1.04 & 0.04 \\
		eajs.2.100.5.ExpUtil    & 12627    & 1349           & \textbf{83}   & 85             & 7 & 0.06 & 0.06 & 1.02 & 0.06 \\
		echoring.MaxOffline1    & 104892   & 48765          & \textbf{934}  & 970            & 94 & 0.02 & 0.02 & 1.04 & 0.02 \\
		elevators.a-11-9        & 14742    & 6790           & 8163          & \textbf{5555}  & 2756 & 1.2  & 0.82 & 0.68 & 1.2  \\
		exploding-blocksworld.5 & 76741    & 39436          & \textbf{2490} & 3635           & 1346 & 0.06 & 0.09 & 1.46 & 0.06 \\
		firewire\_abst.3.rounds & 610      & 51             & \textbf{12}   & \textbf{12}    & 0 & 0.24 & 0.24 & 1    & 0.24 \\
		ij.10                   & 1013     & \textbf{415}   & 645           & 453            & 222 & 1.55 & 1.09 & 0.7  & 1.55 \\
		pacman.5                & 232      & 440            & \textbf{21}   & \textbf{21}    & 0 & 0.05 & 0.05 & 1    & 0.05 \\
		philosophers-mdp.3      & 344      & 251            & \textbf{195}  & 203            & 5 & 0.78 & 0.81 & 1.04 & 0.78 \\
		pnueli-zuck.5           & 303427   & \textbf{59217} & 85685         & 72192          & 26941 & 1.45 & 1.22 & 0.84 & 1.45 \\
		rabin.3                 & 704      & 301            & \textbf{55}   & 58             & 0 & 0.18 & 0.19 & 1.05 & 0.18 \\
		rectangle-tireworld.11  & 241      & 259            & \textbf{240}  & \textbf{240}   & 0 & 0.93 & 0.93 & 1    & 0.93 \\
		triangle-tireworld.9    & 48    & 38             & \textbf{13}   & \textbf{13}    & 0 & 0.34 & 0.34 & 1    & 0.34 \\
		wlan\_dl.0.80.deadline  & 189641   & 6591           & \textbf{1684} & 1824           & 199 & 0.26 & 0.28 & 1.08 & 0.26 \\
		zeroconf.1000.4.true & 1068            & 520          & \textbf{41} & 44            & 1 & 0.08 & 0.08            & 1.07           & 0.08 \\
\midrule
\multicolumn{6}{c}{Geometric means} 			&	0.27 &	0.23	&	0.84	&	0.27\\
		\bottomrule    
	\end{tabular}
\end{adjustbox}
\label{table:nodes-comparison}
\end{table*}
